SoK: Tools for Game Theoretic Models of Security for Cryptocurrencies

Cryptocurrencies have garnered much attention in recent years, both from the academic community and industry. One interesting aspect of cryptocurrencies is their explicit consideration of incentives at the protocol level. Understanding how to incorporate this into the models used to design cryptocurrencies has motivated a large body of work, yet many open problems still exist and current systems rarely deal with incentive related problems well. This issue arises due to the gap between Cryptography and Distributed Systems security, which deals with traditional security problems that ignore the explicit consideration of incentives, and Game Theory, which deals best with situations involving incentives. With this work, we aim to offer a systematization of the work that relates to this problem, considering papers that blend Game Theory with Cryptography or Distributed systems and discussing how they can be related. This gives an overview of the available tools, and we look at their (potential) use in practice, in the context of existing blockchain based systems that have been proposed or implemented.

==> alexstuff.tex <==
The basic primitives of Game Theory are games and the solutions to those games.
The simplest way to characterize a game is by defining a tuple $(N,A,P)$ where $N$ denotes the set of players, $A$ denotes the set of actions available to the players, and $P$ the payoff function for each player, usually a utility function that maps actions to values.
Players play strategies, which map a players local state to actions, and receive payoffs corresponding to their utility function.
The tuple of strategies selected by each player is called the \textit{strategy profile} of the game.
A solution concept for a game is a rule that predicts how the game will play out.
Games come in many shapes and forms as constraints on the players and their information, beliefs, actions and utilities are added or removed (among other things), and we will now introduce the types of games that are most relevant to the topic of \textbf{TITLE TOPIC HERE}

\paragraph{\textbf{Normal form games}}
Games in which players move simultaneously are generally described as \textit{normal form games}, which can be represented as a matrix that contains the players strategies and payoffs for each strategy.
\alex{Figure: example e.g., prisoner's dilemna which is interesting because that equilibrium in theory does not happen in practice for the repeated form}
In this type of game, players are assumed to know the strategies and payoffs available to the other players (i.e., they have \textit{complete} information).
Accordingly, they can make a rational choice of strategy that maximises their payoff given all the strategies that others might play.

Given this setting, one can solve the game by evaluating the optimal choice of strategies for the players.
A player's strategy is said to be (strictly) dominant if the payoff associated to it is (strictly) greater than the payoff associated with any other strategy available to the player, no matter what other players play.
This is enough to solve many simple games, but is not satisfying if we are concerned with players deviating i.e., changing their strategies.
In this case, we desire the notion of equilibrium, where no player is expected to deviate from their strategy no matter what other players do.

An example notion of equilibrium is the famous \textit{Nash equilibrium}.
In a game involving $n$ players with corresponding strategy sets and pay-off functions, a strategy profile is a NE for the game if no unilateral deviation by any single player results in a greater pay-off for that player.
More formally, a NE is expressed in the following way.
\begin{definition}[Nash equilibrium]
\end{definition}
An important result is that a Nash equilibrium always exists for games of this form with a finite set of actions, and many can exist in practice.

\paragraph{\textbf{Extensive form games}}
In practice, many games involve multiple rounds of play with moves made sequentially by players, as in chess for example.
These are generally described as \textit{extensive form} games, which can be represented in a tree form that represents the possible sequences of actions in the game.
Going from a normal form game to an extensive form games requires specifying an ordering of play, payoffs as a function of moves, information sets at (the moves that could have taken place given what a player has observed), and a probability distribution over Nature's moves (moves by players with no strategic interest in the game's outcome e.g., a dealer).

When considering the tree representation of the game, one can find \textit{subgames} i.e., subsets of a game that have an initial node such that it is the only member of its information set, its successors are in the subgame, and the nodes in the informations sets of the subgame are in the subgame.
Subgames are very relevant because they allow us to define a \textit{subgame perfect equilibrium} (SPE), a refinement of a Nash equilibrium that eliminates Nash equilibria involving irrational subgame behavior.
As in the case of a NE, at least one SPE is guaranteed to exist for a finite extensive form game, and we define them as follows:
\begin{definition}[Subgame perfect equilibrium]
A strategy profile is a subgame perfect equilibrium if it represents a Nash equilibrium of every subgame of the original game.
\end{definition}

SPE are usually determined through the use of backwards induction, by starting from the last actions of the game (the leaves of the tree) and going backwards in a way that maximises the final player's utility, then doing the same for the penultimate player and so on, taking into account he optimal moves previously determined for other players.
The remaining strategies are the set of SPE of the games.

In some cases, a path in the tree representing the game might go on forever, making it hard to check whether a strategy profile is a SPE.
One way of dealing with this is to apply a \textit{single deviation test} by considering a strategy profile, picking a stage in the game and a player that moves at that stage.
The chosen strategy profile fixes the moves of the other players at the chosen stage and in the following game.
The chosen player for the stage has fixed moves in future stages of the game , but has a choice at this stage i.e., it is allowed to deviate from the chosen strategy profile once.
If it can move in a way that gives a higher payoff than the strategy profile, then the strategy profile fails the test as the player has an incentive to deviate so the strategy profile is not a SPE.

The  \textit{single deviation principle} formally relates the idea of a SPE to the single deviation test.
It states that a strategy profile of a finite extensive form game, a strategy profile is a SPE if and only if it passes the single deviation test at every stage for every player.
\alex{COuld define formally inside a def environment if space allows, see \url{https://ocw.mit.edu/courses/economics/14-12-economic-applications-of-game-theory-fall-2012/lecture-notes/MIT14_12F12_chapter11.pdf}}

\paragraph{\textbf{Incomplete and imperfect information}}
So far, we have assumed that players have complete information about the game they are in, but this is not always true in realistic systems.
A game where information sets have more than one member i.e., players do not always know exactly what has taken place earlier in the game, is said to have \textit{imperfect information}.
In the case where players do not know exactly the \textit{type} of the other players, which determines their payoff function, the game is said to have \textit{incomplete information}.

Imperfect and incomplete extensive form games can be related by having Nature make the first move in the game and randomly assign types to players, turning an incomplete game into an imperfect game as different outcomes of Nature's initial move are possible.
The players then have a probability distribution over the the types of other players\footnote{Formally speaking, the probability distribution is over the set of states of Nature, which are mapped to player types.}.
The beliefs of players are expressed as conditional probabilities of a history in an information set, given the information set.
Players can then update their beliefs when they gain new information according to Bayes' theorem, leading games of this form to be described as \textit{Bayesian games}.
Beliefs 
A collection of beliefs is called a \textit{belief system}, which paired with a strategy profile form an \textit{assessment}.

Now that we do no longer have perfect information, we must leave behind some existing solution concepts.
The lack of perfect information means that players cannot always tell which subgame they are in, so a SPE is no longer possible.
Players now also think about expected payoffs, so the standard definition of a NE is also no longer appropriate, but we can define a \textit{Bayesian Nash equilibrium} (BNE) analogously by replacing the utility functions with expected utilities.
This does not, however, take into account the beliefs of the players that now have to be considered.
To alleviate this problem, we can further refine the idea of a NE by considering assessments and defining a \textit{perfect Bayesian equilibrium} (PBE) with the following requirements.
First, the assessment should be \textit{sequentially rational} i.e., at every information set the player that moves maximises his expected utility given his beliefs and that other players will play according to the strategy profile in the continuation of the game.
Second, beliefs for information sets on the equilibrium path (of the tree representation) should always be derived using Bayes' rule and those not on the path should be derived using Bayes' theorem whenever possible.

Going further, we can refine the idea of a PBE and define a \textit{sequential equilibrium} which requires an assessment that is sequentially rational and \textit{consistent} i.e., given any information set reached with positive probability (according to the strategy profile) the beliefs at that information set are derived using Bayes' rule and the strategy profile.
This gives a slightly stronger equilibrium due to the stricter constraint on the beliefs.

\alex{Maybe mention something about repeated games?}

\subsubsection{Mechanism design and implementations}


==> app-papers.tex <==
%!TEX root = main.tex
\subsection{List of Papers}
\renewcommand{\arraystretch}{1.5}
{\footnotesize
\begin{tabular}{p{1.3cm} | p{6.5cm}}
\toprule
    % ============= theme 1 ============= %
    \textsc{Crypto and GT} & 
    \cite{butwhy}, 
    \cite{rationalcrypto}
    \cite{rationalcrypto2},
    \cite{rationalcrypto3},
    \cite{rationalcrypto4},
    \cite{rationalityandadversarial},
    \cite{rationalsecretsharing},
    \cite{gt-secure-computation},
    \cite{idealmechanismdesign},
    \cite{Halpern:2004:RSS:1007352.1007447},
    \cite{Fischer1990AnAO}
    \cite{multiparty-computation-game-theory},
    \cite{distributed-computing-game-theory},
    \cite{barational},
    \cite{barprimer},
    \cite{theoryofbargames},
    \cite{selfishmeetsevil},
    \cite{leader-election-gt}\\
    
    % ============= theme 3 ============= %
    \textsc{GT meets DS} & 
    \cite{Feigenbaum:2002:DAM:570810.570812},
    
        % ============= theme 4 ============= %
    
    \cite{acalltoarms},
    \cite{rationalconsensus},
    \cite{DBLP:journals/corr/HalpernPS15} \\


\bottomrule
\end{tabular}
%\caption{List of all paper read for this SoK.}
%\label{tab:list_of_papers}
%\end{table}
}

==> discussion.tex <==
%!TEX root = main.tex
\section{Discussion}\label{sec:discussion}
% \begin{itemize}
% \item Explain how all the solution concepts relate to each other
% as well as different assumptions associated with each of them.
% \item Explain how this could be/have been applied, for example to bitcoin/blockchain
% \item what is missing
% \end{itemize}
\saraha{add here:
In this paper, we reviewed many different concepts and models.
Most of them however are complementary and coul be used in conjunction.
For example the BAR model simply suggests the different types of players
that could be considered and would go well with
other concepts like robustness.
which one are complimentary of each other, which one are not?}

% The interest in blockchains has given an impactful application for
% the theory bridging Game Theory and Computer Science.
% However, most of the research done in that field before the apparition of
% Bitcoin seems to be unused or underused in the blockchain community.

% how all the concepts defined previsouly
%could be used, for example in the blockchain
%community or elsewhere.% (Section~\ref{sec:discussion-use}). %, and highlight what is missing 
%in this space and open problems (Section~\ref{sec:discussion-futurework}).

% \subsection{Relation between different concepts}
% \label{sec:discussion-relation}
% \saraha{change this paragraph, put the 'next concept' instead: covert adversary,
% bar , etc}
% \saraha{this paragraph is redundant from background. not sure it makes
% sense here, let's see}
% Both Mechanis Design, Cryptography and DS are about understanding the collaborative
% interactions among parties that do not trust each other and can have conflicting
% interests, as well as
% designing and analyzing protocols for parties in such situations.
% They have, however, different goals and formalisms.


% \subsubsection*{Aims} 
% % Mechanism design-> solution concepts (e.g., NE), optimal solution
% % crypto, ds->security
% Cryptography aims to
% ``protect'' honest players against the worst possible adversaries (according to the hardness assumptions) with respect to some security properties (e.g., secrecy and correctness).
% In the simulation paradigm, the security of a protocol is captured by
% defining an ideal functionality (how the protocol should behave if
% there was a trusted party enforcing it). The ideal functionality is somehow comparable to the mediator in GT.
% Cryptographers then
% need to show that there is a simulator that emulates the protocol
% in some ideal world where a trusted third party executes the functionality.
% % Incentives are not consider in traditional DS or cryptography but
% % some work has been done to incorporate them and bridge GT and Computer Science.
% % We present them in the next sections.
% Mechanism Design, on the other hand does not consider any privacy and correctness concerns, it is concerned with implementing a solution concepts
% and reaching an optimal state. Designing rules that will naturally lead to behaviours with
% the desired properties.

% \subsubsection*{Underlying assumptions}

% Mechanism design considers the existence of a central party (the center)
% that is trusted to enforce the mechanism.
% Cryptography and DS on the other hand do not assume any trusted third party.
% They usually have some complexity assumptions (e.g., discrete log is NP-hard)
% and some communication assumptions (e.g., synchronous or asynchronous network).

% Thus, in cryptography and DS everything is possible,
% in term of action, given the computational and communication assumptions.
% In GT the set of actions is usually more restricted. i.e the mediator decides
% the set of actions.
% Cryptography and distributed system relies on the honesty of at least some players.


% On of the difficulty when doing security is that it is hard
% to think about all the possible strategies that an adversary
% may try and use to attack the system.
% % In cryptography, simulation-based proofs are useful
% % because they allow to consider every possible
% % adversarial behaviour as opposed to GT where the set of actions is usually
% % finite or at least well defined.
% In cryptography, simulation-based proofs solve this problem
% because they allow to consider every possible
% adversarial behaviour.
% Again the intuition is that whatever actions the adversary can do
% in the real world, it can be simulated in the ideal world.
% Since the ideal world is by assumption secure then the real
% world must be secure as well.
% The field of Rational Cryptography uses similar techniques
% but while using a rational adversary and simulating its utility
% function. This framework is however limited
% as it does not consider irrational adversaries that are
% paramount when designing secure decentralized systems.

% In DS, Byzantine players are allowed to take arbitrary
% deviations from the protocol, given the underlying communication and network assumptions.
% The systems are however often very complex and even if they
% provides proofs, some flaws are being discovered, years later~\cite{revisitingfastpbft}.
% \saraha{need to  re-write this better}
% % Some allegedly secure systems with proofs are being broken~\cite{revisitingfastpbft}
% % Complex systems, hard to know is something's broken
% % The use of Game Theory is more widespread in the Distributed Systems
% % community than, for example, Cryptography
% % with designs like selfish routing etc.
% % \saraha{add}

% In GT there is no real adversary, just selfish agents. Their sets of
% action is usually limited by the definition of the game.
% Proofs are then different due to stronger assumptions.
% \saraha{what extensions have been made?}


% \subsection{How can these concepts be used}
% \label{sec:discussion-use}
% \saraha{correlated equilibrium somehwere?}
%take every useful concept and say where it has and should/coul be applied.
We now discuss the ways in which the concepts presented in the previous sections could be used.
%First, we have already argued that NE are too weak as a solution concepts for blockchain protocols because they do not consider coalitions or fully malicious players.
%We argue that $(k,t)-$robustness, presented in Section~\ref{sec:dsgt}, is a better fitted solution concept.
First, we have already argued that $(k,t)-$robustness, presented in Section~\ref{sec:dsgt}, is a better fitted solution concept than NE for blockchain protocols because they do not consider coalitions or fully malicious players.
So far this concept has only been used in Fant\^omette~\cite{fantomette} and a preliminary version of Solidus~\cite{solidus}.

Even though it does not consider malicious adversaries, the RPD framework would still work well in the case of payment channels.
In that case, even if an adversary is fully malicious, they could cheat but if they do so the other party will then be able to claim all of their deposit.
In that case the non-cheating party would end up in a better situation, as they would earn even more.
The RPD model is then perfectly adapted as even an irrational adversary cannot harm an honest player.
Moreover, as it is clear how the adversary can cheat (by broadcasting an old transaction), RPD is useful since it provides a relaxed functionality that specifically allows bad behaviour.
%A cost will be associated with this bad behavior e.g., in the case of payment channels the whole deposit of the cheating player will be taken away. 
%Furthermore, formal models that have been proposed for payment channels are already based on the UC model~\cite{sprites,statechannels}, thus extending them to consider the RPD would not be as hard as the tedious part is very often the UC emulation.

Alongside RPD, we also presented work on BMG, which could be usefully applied to cryptocurrencies given that many situations are modeled as games involving computations e.g., mining.
The equivalence theorems between secure computation and game theoretic implementations also give a direct connection to standard notions of security, although they are given for specific variants of implementations and secure computation that may not match those required in practice. Further results in this domain could however prove very useful.
As the cryptographic side is founded on the ideas that also form the basis of simulation based Cryptography and UC model it may be possible to connect both frameworks.
%This result is convenient, in that it allows us to show only that there is a secure computation or an implementation and have the second side for free, which could be a practical way of avoiding the complexity of proofs involving both Cryptography and Game Theory.
%The results of Halpern and Pass are also given in the case of specific variants of implementations and secure computations, so it is not necessarily obvious that these match those required in practice, but further results in this direction could change this.
The given example of a game that deals with covert adversaries also shows that this can be used in practice, even if it is not clear that applying this method will produce more efficient solutions to problems.

%However, there are certainly problems in modelling aspects of cryptocurrencies that are more easily defined as games

%Most fo the work consists in proving the emulation part.
%Furthermore, ideas used on the work of selfish routing could be used in routing payment network.
% The Fear factor -- where the presence of irrational players incentivizes rational players
% to follow the rules-- could be leveraged in some scenario to improve some system.
% For example in Tor~\cite{tor}, players can be incentivized to run nodes based on the assumption that some other nodes are irrational and are trying to attack the network.
% Indeed, the more nodes the more secure the network is.
% Otherwise there is no incentive to run a Tor node. Indeed if a rational players assumes that every other players runs a node, then their privacy is protected even if they do not do so.
% \alex{Eh}
% \saraha{remove tor and talk about fear factor with spv, if everyone is rational verifying blocks is not
% an equilibrium cf verifier dilemma but fear of irrational players may incentivize to verify blocks}
% Thus running a node is not a Nash Equilibrium.
In Bitcoin, the blockchain takes up a few hundred gigabytes of space.
Most users do not run a full node that requires storing the whole blockchain and verifying every block, instead they use light clients (i.e., simplified payment verification, SPV) that store only hashes of the blocks and connect to full nodes that they must trust, which is not ideal.
%Placing trust in another node is not ideal in a decentralized system.
This problem can be compared to the problem of free riding in P2P file systems, and ideas from that context could be used to help incentivize users to run full nodes.
In the same vein, Bitcoin's PoW is comparable to total effort and best shots public goods, discussed
in Section~\ref{sec:dsgt}.
The security of the system depends both on the total
hashrate of the network (it is less expensive to attack a network with a smaller hashrate)
and on the maximum hashrate of a single player or pool (as a single player
detaining half or close of the total hash power represents a threat for the system).

The fear factor, introduced in Section~\ref{sec:dsgt}, could also be used. As explained
in Section~\ref{sec:blockchains}, with the verifier's dilemma~\cite{verifierdilemma},
verifying the content of blocks is not an equilibrium, %  when all the participants are rational.
however, some users may be motivated to do it by fear that others will not.
For example, a user may choose to run a full node rather than an SPV, which would improve the overall system.
Under this assumption, an equilibrium may be reachable.

The Price of Malice could also inspire new measures that quantify the trade-off between blockchain and traditional consensus protocols.
Blockchain-based systems are intended to be more scalable as they are meant to handle open participation, compared to classical consensus that requires the many messages to be exchanged, but in the case of Bitcoin this comes at the price of PoW so there is an incurred economic cost.

As differentiating between malicious behavior and genuine latency is hard, especially in PoS systems, the Price of Unaccountability may be a useful to evaluating this. Since this problem is related to that of Hidden actions, we could also explore using the principal-agent model there as presented in Section~\ref{sec:dsgt}.

Cryptocurrencies are the first family of distributed systems that includes creation of new money 
so transfer functions could be used here e.g., to find an optimal reward scheme. Briefly, in order to provide the incentives necessary to make efficient choices, it may be
necessary to tax or subsidize various individuals.
%e.g., add a financial punishment.
Adjustments are made by a transfer function $t:\Theta\rightarrow\mathbb{R}^n$,
where $t_i(\theta)$ represents the payment that player $i$ receives (if $t_i(\theta)<0$)
or make (if $t_i(\theta)<0$). 
%One example of transferable utility function is quasi-linear utility function which has the form:
%%$u_i(\vec{\theta},\theta_i,d,t)=v_i(d(\vec{\theta}),\theta_i)+t_i(\vec{\theta})$
%$u_i(\vec{\theta},t)=v_i(\vec{\theta})+t_i(\vec{\theta})$
%where $v_i$ is the agent's valuation for the outcome.
Could we find an equivalent to the revelation principle here, for example by using blockDAGs that reveal more about the decision making of a player?
% }
% \else{Cryptocurrencies are the first family of distributed systems that includes creation of new money so transfer functions could be used here e.g., by the designer to find the optimal reward scheme of a cryptocurrency.
% Could we find an equivalent to the revelation principle here, for example by using blockDAGs that reveal more about the decision making of a player?}\fi
Another avenue for the design of blockchain based systems could be to investigate implementing direct reciprocity, as opposed to indirect reciprocity, to incentivize good behavior and force miners to cooperate more, as discussed in Section~\ref{sec:dsgt}.
% \subsection{Figure}
% We plotted a graph that represents the cross-citation between the papers
% that we reference here, i.e., two papers are linked in the graph if
% one references the other.
% We see in Figure ... that there are three distinct clusters that correspond
% to the different communities considered here.

With regards to consensus protocols, something that is missing from the blockchain literature is a general framework
for comparing and evaluating them.
Many operate under very different assumptions and the outcome would be greatly different when changing those.
For example, Algorand does not consider
rational players, which is a much stronger assumption than other protocols, and it is not clear how rational players would behave in this setting.
Others do not consider the centralization problem or compounding of wealth.

Finally, it could be useful to develop a framework for games with a large amount of players.
While the overall goal of a cryptocurrency is to be decentralized at a large scale with a very large amount of independent nodes, our current models usually only treat games with a well defined and small amount of players, which may not capture the behaviour that a truly large scale decentralised system would observe due to added complexity.
Here, tools from complexity economics and the study of dynamical systems may be useful.


\saraha{fairness vs equitability
type of incentives (economic non economic)
read again discussion from spw}



==> economicsofblockchains.tex <==
Economics of blockchains

Suggests two approaches to
economics of blockchain: innovation-centred and governance-centred. 

==> prelim.tex <==
%!TEX root = main.tex
\section{Background}
\label{sec:prelim}

In this section we briefly introduce game theoretic tools that are mentioned throughout the paper such as solutions concepts and mechanism design.
For a complete introduction to Game Theory, the reader is invited to look at any of the books  (or other resources) on the topic~\cite{gametheoryowen,jackson}.
For the sake of exposition we omit to cover concepts that are relevant e.g., Pareto efficiency and the single deviation test, as these do not appear in the papers we mention.
We also discuss the interface between Game Theory and Cryptography and Security in practice, from how both areas define their agents to the models used to reason about them.
We then give a brief introduction on Distributed Systems and cryptocurrencies.

% Here we give some background on different concepts
% of Game Theory (GT), Cryptography and Distributed Systems (DS).
% We refer the reader to ... for a comprehensive litterature review.

% \begin{itemize}
% \item solution concepts in GT like NE, strategyproofness, revelation principle, (sequential equilibrium,)
% social welfare maximization, individual rationality use \url{https://www.cs.cmu.edu/~sandholm/cs15-892F15/Rahul-thesis.pdf}
% \item safety liveness in DS
% \item UC and game proof in crypto
% \end{itemize} 



\subsection{Game Theory and Mechanism Design}
\subsubsection{Games and solution concepts}
% We refer the reader to~\cite{jackson} for a more complete background
% on Game Theory and Mechanism Design.
A game is defined by a set of $n$ players and a set of actions
for each player $(A_1,\cdots,A_n)$.
A strategy for player $i$, denoted $\strategy_i$, is a function from $i$'s local state to actions $A_i$. 
We denote $\strategyset_i$ the set of all possible strategy for player $i$.
We denote $\vec{\strategy}=(\strategy_1,\cdots,\strategy_n)$ the joint strategy of all players
and $\vec{\strategy}_{-i}=(\strategy_1,\cdots,\strategy_{i-1},\strategy_{i+1},\strategy_n)$.
We denote $u_i(\vec{\strategy})$ player's $i$ utility when $\vec{\strategy}$ is played.
Players may be of different types, which are denoted $\theta_i$ for player $i$.

Game Theory uses solution concepts in order to predict the outcome of a game, the most well known is the \textit{Nash equilibirum} (NE).
A strategy $\vec{\strategy}^{NE}$ is a Nash equilibrium if given that all the other players follow $\vec{\strategy}^{NE}_{-i}$, player $i$ is better off playing $\strategy^{NE}_i$ as well.
More formally, for all players $i$ and all strategies $\strategy_i$: $u_i(\strategy_i^{NE},\vec{\strategy}_{-i}^{NE})\ge u_i(\strategy_i,\vec{\strategy}_{-i}^{NE})$. Note that multiple NE can exist for a given game.

\paragraph{\textbf{Extensive form games}}
In practice, many games involve multiple rounds of play with moves made sequentially by players, as in chess for example.
These are generally described as \textit{extensive form} games, which can be represented in a tree form that represents the possible sequences of actions in the game.
Going from a normal form game to an extensive form games requires specifying an ordering of play, payoffs as a function of moves, information sets (the moves that could have taken place given what a player has observed), and a probability distribution over Nature's moves (moves by players with no strategic interest in the game's outcome e.g.,  a dealer). 

When considering the tree representation of the game, one can find \textit{subgames} i.e.,  subsets of a game that have an initial node such that it is the only member of its information set, 
its successors are in the subgame, and the nodes in the informations sets of the subgame are in the subgame.
Subgames are very relevant because they allow us to define a \textit{subgame perfect equilibrium} (SPE), a refinement of a Nash equilibrium that eliminates Nash equilibria involving irrational subgame behavior.
As in the case of a NE, at least one SPE is guaranteed to exist for a finite extensive form game, and we define them as follows:
a strategy profile is a subgame perfect equilibrium if it represents a Nash equilibrium of every subgame of the original game.


% SPE are usually determined through the use of backwards induction, by starting from the last actions of the game (the leaves of the tree) and going backwards in a way that maximises the final player's utility, then doing the same for the penultimate player and so on, taking into account the optimal moves previously determined for other players.
% The remaining strategies are the set of SPE of the games.

% In some cases, a path in the tree representing the game might go on forever, making it hard to check whether a strategy profile is a SPE.
% One way of dealing with this is to apply a \textit{single deviation test} by considering a strategy profile, picking a stage in the game and a player that moves at that stage.
% The chosen strategy profile fixes the moves of the other players at the chosen stage and in the following game.
% The chosen player for the stage has fixed moves in future stages of the game , but has a choice at this stage i.e.,  it is allowed to deviate from the chosen strategy profile once.
% If it can move in a way that gives a higher payoff than the strategy profile, then the strategy profile fails the test as the player has an incentive to deviate so the strategy profile is not a SPE.

% The  \textit{single deviation principle} formally relates the idea of a SPE to the single deviation test.
% It states that a strategy profile of a finite extensive form game, a strategy profile is a SPE if and only if it passes the single deviation test at every stage for every player.

\paragraph{\textbf{Incomplete and imperfect information}}
So far we have assumed that players have complete information about the game they are in, but this is not always realistic.
A game where players do not always know exactly what has taken place earlier in the game, is said to have \textit{imperfect information}.
In the case where players do not know exactly the \textit{type} of the other players, which determines their payoff function, the game is said to have \textit{incomplete information}.

Imperfect and incomplete extensive form games can be related by having Nature make the first move in the game and randomly assign types to players, turning an incomplete game into an imperfect game as different outcomes of Nature's initial move are possible.
The players then have a probability distribution over the types of other players. (Formally speaking, the probability distribution is over the set of states of Nature, which are mapped to player types.)
The beliefs of players are expressed as conditional probabilities of a history in an information set, given the information set.
Players can update their beliefs when they gain new information according to Bayes' theorem, leading games of this form to be called \textit{Bayesian games}.
A collection of beliefs is called a \textit{belief system}, which paired with a strategy profile is an \textit{assessment}.

Now that we do no longer have perfect information, we must leave behind some solution concepts.
The lack of perfect information means that players cannot always tell which subgame they are in, so a SPE is no longer possible.
Players now also think about expected payoffs, so the standard definition of a NE is no longer ideal but we can define a \textit{Bayesian Nash equilibrium} (BNE) analogously by replacing utilities with expected utilities, although we usually still refer to them simply as utilities. 
This does not, however, take into account the beliefs of the players that now have to be considered.
% To alleviate this problem, we can further refine the idea of a NE by considering assessments and defining a \textit{perfect Bayesian equilibrium} (PBE) with the following requirements.
% First, the assessment should be \textit{sequentially rational} i.e.,  at every information set the player that moves maximises their expected utility given their beliefs and that other players will play according to the strategy profile in the continuation of the game.
% Second, beliefs for information sets on the equilibrium path (of the tree representation) should always be derived using Bayes' rule and those not on the path should be derived using Bayes' theorem whenever possible.

Going further, we can define a \textit{sequential equilibrium} which requires an assessment that is sequentially rational and \textit{consistent} i.e.,  given any information set reached with positive probability (according to the strategy profile) the beliefs at that information set are derived using Bayes' rule and the strategy profile.
This gives a slightly stronger equilibrium due to the stricter constraint on the beliefs.

\subsubsection{Correlated Equilibria}
NE and BNE are very powerful tools use widely in GT, however they also have a lot of
drawbacks (e.g., computing it is not tractable~\cite{daskalakis2009complexity}) and do not yield to the
obvious best general outcome (see the famous prisoner's dilemma for example~\cite{sep-prisoner-dilemma}).
For this reason some other solution concepts exist.
One notable is
the \textit{correlated equilibrium}.
The intuition behind a correlated equilibrium can be interpreted as follows:
let's assume that there exists a public signal that tells players what
to play; based on the information they receive players can make inference
about the move that the other players are going to play.
For example a public signal could be a traffic light. If a player sees
a red light they can assume that another player on another line will
see a green light and thus that their best decision is to stop at the intersection.
Thus in a correlated equilibrium, each players choose their actions
according to information given by the public signal. The role of the public signal
is usually to help players achieve the optimal outcome of the game.

\subsubsection{Mechanism design (MD) and Implementations}
While Game Theory is typically about understanding the behavior of players in a given game, systems are usually designed and implemented with a goal in mind e.g., preventing double spending in cryptocurrencies.
To achieve this, our goals can be expressed as a social choice function (SCF), a function that given the preference (or types) of all players outputs an outcome.
For example, in a voting system, given all the ranked preferences of voters, a SCF will
choose a candidate.
% We can also define a social welfare function (SWF) as a function that given the preference of all players outputs a global preference. For example, given all the ranked preferences of voters, a SWF will
% output a ranked list of candidates.

Once we have a target outcome in mind, the idea is to make sure that %it happens.
the incentives are designed in a way such that selfish players reach this outcome.
In some ways, this can be thought of as reversing the basic idea of Game Theory, designing a game that leads to a specific outcome.

To do this, we use a mechanism that maps the action profile of players to a distribution over outcomes.
A mechanism $M$ is then said to implement a SCF $f$  if $M(C_M(\vec{u}))=f(\vec{u})$, where
$\vec{u}$ is the vector of all of the players utility functions and
$C_M(\vec{u})$ represents all strategy vectors that could reasonably result from selfish behavior.
Informally the previous equality means that whatever selfish strategy players
choose, the outcome of the game will correspond to the SCF.
The solution concept is supposed to reflect reality, in the sense that when it holds, players' selfish strategies lead to the desired outcome.
For example in a voting system we would like to design a system where given all the preferences
of the players, the one chosen by the SCF is elected, one way to do this is to incentivize players to
report their truthful preferences.
A mechanism can also be viewed as a protocol, with the corresponding game being thought of as having the protocol as the recommended strategy, and deviations from the protocol as other possible strategies.

It must be pointed out that doing this in practice is not always easy, as experimental Game theory reveals. Gneezy and Rustichini~\cite{gneezy2000fine} looked at the effects of implementing incentives at a nursery in order to reduce the rate at which parents collected their child late.
% \alex{Could also mention the field of experimental game theory that looks at confirming theoretical results in experiments, as this is something that's often neglected in discussions.}
This was done by punishing late parents with a fine, which intuitively should motivate parents to arrive on time. Instead, parents interpreted the fine as a way of paying for extra childcare, and started coming even later.
Furthermore, once the fine was removed as it was counter productive, the parents behavior did not revert back so the system had in fact been irreversibly damaged.

%In a sense, a mechanism can also be viewed as a protocol, with the corresponding game being thought of as having the protocol as the recommended strategy, and deviations from the protocol as other possible strategies.

% GT usually focuses on predicting and analysing the behavior of players in a game,
% the subfield of Mechanism Design is often refered to as reverse GT
% as it is concerned with the question of how to design a game such
% that players will behave in a way that leads to an optimal situation.
% More formally a mechanism defines a pair (A,M) where A is the set of actions
% available to the players and M maps eacg action profile to a distribution
% over outcomes. For example in the voting case, the designer would chose
% the set of actions as being, for example, ranking all the candidates and the
% We give a formal definition in the glossary in the appendix.


% Let us denote L the set of linear order on outcomes (that is L is
% isomorphic to the set of permutations on O).
% The preferences of player $i$ are then given by $\succ_i\in L$,
% where $o_1\succ_i o_2$ means that player $i$ prefers outcome $o_1$ to $o_2$.
% A function $F:L^n\rightarrow L$, that given the preferences of all players outputs
% a global preference is called a social welfare function.
% A function $f:L^n\rightarrow O$, that given the preferences of all players outputs 
% an outcome is called a social choice function (SCF).

% A social choice function is strategyproof if $u_i(f(u))\ge u_i(f(u|^iv))$
% for all $i$ and $v\in L$ and where $(u|^iv)_i=v$ and $(u|^iv)_i=u_j$. The idea is that
% players are better off declaring their real utilikty function.

% In mechanism design the objectives are to implement a mechanism that
% satisfies certain properties
%either strategy proofness, or budget-balance etc
% A mechanism implements a SCF $f$ if $M(C_M(u))=f(u)$, where $C_M(u)$ represents all strategy
% vectors that could reasonably result from selfish behavior and is called the solution concept.
% The solution concept is supposed to reflect reality, in the sense that when it holds, player's selfish strategies lead to the desired outcome.
% For example if the desired outcome is a NE, then we define a bayes-Nash implementation
% as follows:
% % \begin{definition}[Bayes-Nash implementation]
% % Given a Bayesian setting $(N,O,\Theta,p,u)$, a mechanism (A,M) is an implementation
% % in Bayes-Nash equilibrium of a social choice function f (over N and O) if there exists a Bayes-Nash equilibirum
% % of the game $(N,A,\Theta,p,u)$ such that for
% % every $\theta\in\Theta$ and every action profile $a\in A$ that can arise given
% % type profile $\theta$ in this equilibrium, we have that $M(a)=f(u(\cdot,\theta))$.
% % \end{definition}

% \begin{definition}[Bayes-Nash implementation]
% A mechanism M is an implementation
% in Bayes-Nash equilibrium of a social choice function f if there exists a Bayes-Nash equilibrium
% of the game such that for
% every $\theta\in\Theta$ and every action profile $a\in A$ that can arise given
% type profile $\theta$ in this equilibrium, we have that $M(a)=f(u(\cdot,\theta))$.
% \end{definition}

A very important result in MD is the revelation principle %~\cite{jackson}
that states that any social choice function that can be implemented
by any mechanism can be implemented by a direct truthful mechanism. (A mechanism is direct if players
need only reveal their type/utility function to the designer of the game and truthful if players'
best strategy is to reveal their true type.)

\alex{Do we talk about transferable utilities much later on?}



% Game Theory often assumes the existence of a trusted mediator or center
% to enforce the game's rules.
% This is unrealistic or hard to implement in practice.
% Cryptography and Distributed System solve this problem.


\subsection{Agents in Game Theory and Security}
Both Game Theory and Security deal with the interaction of agents in a given setting, but they differ noticeably in the way they model these agents. 
On the other hand, security proofs are often game based, which points to some similarities.

Security scholars deal with \textit{adversaries}, agents that aim to circumvent or otherwise break a security property of the system. 
The value that an adversary attaches to their success is not usually given, as security should ideally be robust to any adversary, although they may have computational limitations.
Game theorists, on the other hand, deal with \textit{rational} (sometimes also called \textit{selfish}) agents.
These assign a value to their goals, and would rather optimize their payoff than achieve an arbitrary goal, but they typically do not have restrictions (e.g.,  computational) like a security adversary would.

In practice, this translates to different assumptions being used when formally modeling a game or the security of a system.
This makes it difficult to then prove statements that involve security and game theoretic properties.
As both deal with different types of agents, a proof will involve the complexity from both sides and quickly become hard to manage.
This leads to a disjoint treatment of both aspects in works that attempt to cover both.

Despite this, there are nonetheless inherent connections as security often uses game based proofs, although an adversary wins if they have a good enough probability of succeeding in their attack rather than if their utility is high enough. 
But if we assume that the adversary has a high payoff associated with the success of their attack, then we start to recover game theoretic intuition.
Similarly for proofs based on the simulation (ideal/real world) paradigm, some connections are evident.

The idea behind the simulation paradigm first originated in the context of secure computation.
Goldreich et al.~\cite{Goldreich:1987:PAM:28395.28420} introduced the idea of bypassing the need for a trusted third party (i.e., a mediator) in games of incomplete information, by replacing it with a protocol that effectively simulates it such that any information known by players at any step of game is the same as they would have known in an execution of the game involving the trusted third party.
This was then refined by Micali and Rogaway~\cite{micali1991secure} in terms of ideal and secure function evaluation.
The ideal function evaluation corresponds to the evaluation of the function with a trusted third party that receives the private inputs of the parties and evaluates the function before returning the result to each party.
Intuitively, this achieves the best possible result.
The secure function evaluation involves the parties trying to simulate the ideal trusted third party, the protocol used to do so is then considered secure if the parties cannot distinguish between the ideal and secure function evaluations.
This means that the protocol performs close enough to the standard of the ideal function evaluation, and an adversary would not have anything to gain.

Simulation has become a popular tool for cryptographers~\cite{EPRINT:Lindell16}.
In particular, Canetti's Universal Composability Model~\cite{FOCS:Canetti01} expands on these ideas to provide a framework for secure composability of protocols. 
As the UC model is used in some of the work that is covered in Section~\ref{sec:cryptoandgt}, we quickly introduce it here.
Canetti considers an ideal functionality $\mathcal{F}$, an algorithm for the trusted party, that is executed in an instance of the ideal protocol. 
A protocol $\pi$ then UC-realizes an ideal functionality $\mathcal{F}$ if it emulates the instance of the ideal protocol for $\mathcal{F}$.
The protocol $\pi$ UC-emulates a protocol $\phi$ if for any adversary $\mathcal{A}$ there exists an adversary $\mathcal{S}$ (also called the simulator) such that, for any environment $\epsilon$, the output of $\epsilon$ interacting with $\mathcal{A}$ and parties running $\pi$ is indistinguishable from the output of $\epsilon$ interacting with $\mathcal{S}$ and $\phi$.
This builds on the idea of secure function evaluation, where $\phi$ will be the ideal protocol of some ideal functionality $\mathcal{F}$. If the outputs of $\pi$ are then indistinguishable from those provided by $\mathcal{F}$ then we recover Micali and Rogaway's idea of secure computation.
Using this, the UC-model guarantees composability in the sense that if $\pi$ UC-emulates $\phi$, then for any composed protocol $\rho^{\pi\rightarrow\phi}$ UC-emulates $\rho$ i.e., 
if $\rho$ has $\phi$ as subroutine, then replacing calls to $\phi$ by calls to $\pi$ does not change the behavior of $\rho$.
This is formalized with interactive Turing machines (ITM) as model of computation, and allows for parallel and sequential executions of a protocol that is secure.

% simulating the trusted third party required 

% for $n$-player games of incomplete information that required a trusted third party (in other words, $n+1$ players), suggesting it could be replaced by cryptography

% First defined by Goldreich et al.~\cite{Goldreich:1987:PAM:28395.28420} and Micali and Rogaway~\cite{micali1991secure} in the context of secure computation, the idea behind this security model is that there are two worlds.
% The ideal world involves no cryptography, but there is a incorruptible trusted third party (the ideal
% functionality) that receives a players input and outputs a type.
% In a sense, this a purely game theoretic world.
% The real world does not have an ideal functionality, but involves cryptography.
% Security is then achieved if one cannot distinguish between the two worlds, or in other words if the cryptography replaces the trusted third party i.e.,  it is an implementation of the ideal functionality.


% Initiated by the need for private communication and encryption,
% the cryptography field is now concerned with wider problems, like
% %now researcher are doing more complex systems,
% using cryptographic primitives to achieve multiparty
% computation (where parties jointly compute a function over their inputs while keeping
% them private) or secret sharing (where a secret is shared among a set
% of parties, and can only be reconstructed when the shares are aggregated) or
% zero-knowledge proofs (where a prover proves the knowledge of some statement
% to a verifier without revealing any additional properties about that statement).
% Crypto, first secure communication, modern cryptography now much wider,
% especially secure multi-party computation secret sharing zkp etc.

% Cryptography is usually concerned with two types of adversaries:
% semi-honest adversaries, who follow the protocol
% but try to learn more information than intended,
% and fully malicious adversaries, who deviate from the protocol.
% The rest of the parties are honest, meaning that they simply
% follow the protocol.

% To prove security of a cryptographic protocol one usually needs
% to reduce it to a hardness assumption (e.g., the discrete logarithm problem is NP-hard).
% This means that breaking the security of the protocol would imply
% breaking that hardness assumption.
% They are different type of cryptographic proofs: game-based proofs~\cite{introtocrypto,shoup-game} or simulation based~\cite{howtosimulateit}.
% In this paper, all the cryptographic proofs will be based on
% the simulation paradigm.
% The main idea behind simulation-based proofs is to consider an ideal
% world where players have access to an ideal functionality that would take
% their inputs, compute the function to be computed and hand-in each output
% to players respectively.
% The cryptographer then needs to prove that this ideal worl is indistinguishable
% from the real world, i.e.,  where players execute the protocol without
% any trusted authority. The idea being that an adversary, observing or taking
% part in the real worl will learn nothing more than if taking part in the
% ideal worl experiment. Because the ideal world is perfectly secure then this means
% that the real world is also secure.
% One type of proof, that follows from simulation-based ones, is the Universal Composable (UC) security~\cite{uc}.
% UC is an extension from the simulation paradigm that allows for
% composability, meaning that the security is preserved
% even if the protocol is run under concurrent composition of an
% unbounded number of protocol executions (e.g., the protocol is run multiple
% times sequentially or in parallel).
% We will not got into the details of this model but keep a high-level idea
% of the concepts behind it.
%What does it mean to realize a functionality?

% only one we mention in the rest of the paper}
% \subsubsection*{UC Model}
% PT stands for polynomial-time
% define ITM


% A protocol is represented as a system of probabilistic
% interactive Turing machines (ITMs)~\cite{uctuto}, where each ITM represents the program to be run by a party.
% We assume the existence of a trusted third party that obtains the inputs
% from the participants and outputs to each of them their corresponding outputs.
% The algorithm run by this third party is called the \textit{ideal functionality}.
% Emulation means that for any adversary $\adv$ attacking the real  protocol
% execution, there exists an ``ideal-process adversary'' or simulator $\mathcal{S}$
% that causes the outputs of the parties in the ideal process to be the same as
% those in the real execution. In the UC model, an additional adversarial entity,
% the environment, is added. It generates the inputs to all parties, reads all outputs
% and interact with the adversary in an arbitrary way.

% The ideal functionality is modeled as another ITM that interacts
% with the environment and the adversary via a process described below. More specifically, 
% The ideal
% process involves an ideal functionality $\mathcal{F}$, an ideal process adversary (simulator) S, an environment
% $\mathcal{Z}$ with input $z$, and a set of dummy parties $\tilde{P}_1,\cdots,\tilde{P}_n$.
% The dummy parties are fixed and simple ITMs: Whenever a dummy party is activated with an
% input, it writes it on its outgoing communication tape for the ideal functionality $\mathcal{F}$. Furthermore,
% whenever a dummy party is activated due to delivery of some message (from $\mathcal{F}$), it copies this
% message to its output. At the conclusion of a dummy party's activation, the environment $\mathcal{Z}$ is
% activated. The communication by the dummy parties is with the ideal functionality $\mathcal{F}$ only.


\subsection{Distributed Systems (DS)}

A distributed system is a system that consists of a set of connected
components that communicate with each other in order to achieve a common goal.
One important problem is the consensus or Byzantine agreement one where,
informally, the components of the system have to agree on a single value.

DS consider two types of agents, good (i.e.,  agents that follow the protocol) and bad agents that can be of different types (e.g., a \textit{crash fault} where a component halts).
In this paper we will focus on the most general type of fault, Byzantine faults, where a bad agent may act in an arbitrary way.
Traditionally, DS focus on proving two properties: \textit{safety} and \textit{liveness}.
Intuitively, these properties are often summarized as  follows.
Safety means that nothing bad happens and liveness says that something
good eventually happens.

For example, a solution to a consensus problem usually requires three conditions to be met,
agreement (all good agents should agree on the same value), validity (if
all good agents have the same initial value then they should agree on that value),
termination (all good agents should decide on a value).
Agreement and validity fall under safety and termination under liveness.
A system where the safety and liveness conditions are met even
in the presence of Byzantine fault is called \textit{Byzantine fault tolerant}.

A famous solution to the consensus problem in the presence of Byzantine adversaries, is the Practical Byzantine Fault Tolerance algorithm (PBFT)~\cite{pbft} that can tolerate up to a third of the network being Byzantine.
PBFT proceeds in three phases: pre-prepare, prepare and commit.
At each stage each player usually needs to multicast a message to their peers, making the message complexity of this protocol very high
and thus inapplicable to large networks.

Additionally, in traditional Distributed Systems, the set of participants
is not fully open in order to defend against Sybil attacks where an
adversary create many identities to take control of the network.


\subsection{Decentralization, incentives and security}
Because the security of most decentralized systems,
like cryptocurrencies, is linked not only to the security of the protocols, but also to 
%achieving an honest majority of participants, 
having a majority of participants following the rules,
decentralization and incentives have to be considered.

The ideal system does not depend in any way on any single party, which requires it to be decentralized.
Troncoso et al.~\cite{SystematizingDecentralizationandPrivacyLessonsfrom15YearsofResearchandDeployments} give an overview of decentralized systems, defining a decentralized system as ``a distributed system in which multiple authorities control different components and no single authority is fully trusted by all others''.
This highlights the fact that every component of the system should be decentralized, and in particular a single authority distributing its own system (or component) is not decentralized.
This can be hard to achieve in practice, and the level of decentralization of a system should always be looked at critically.
A decentralized system where all important parties are independent but under the jurisdiction of a single government may not truly be decentralized. 
All these independent parties may also depend on a very few hardware manufacturers (or other service providers).

Incentives are key to achieving an honest majority.
Azouvi et al.~\cite{10.1007/978-3-030-03251-7_15} give an overview of the role incentives play in security protocols, including cryptocurrencies.
This highlights the fact that achieving guarantees of equilibria on paper may not be meaningful in practice when the wrong assumptions and models are used.
%, leading to unrealistic results.

What does security mean in this context? Clearly, protocols that are cryptographically secure, and that achieve safety and liveness guarantees are needed, otherwise everything else would not work. 
But if the security of the system also depends on achieving a high enough degree of decentralization, more than standard security properties is required.
%In particular, decentralization relates to the users of the system rather than a protocol in the system. 
In particular, decentralization relates to the participants and their behavior rather than
solely the protocol.
Any decentralized protocol can always be ran in a centralized manner, so it is not enough to design a system that can be used in a decentralized manner. Rather, the requirement is to design a system that is advantageous to use in decentralized manner. 

Doing this naturally requires a better understanding of why users would want to be decentralized rather than try to gain more individual control of the system for themselves, so security is no longer just about the protocol itself, but also about how it can be used and how it is used.


\subsubsection*{Bitcoin and cryptocurrencies}
% Another system that solves the Byzantine agreement problem
% is Bitcoin. In Bitcoin, the assumptions are very different
% from traditional distributed systems~\cite{bano2017consensus},
% as the setting is completely open and permissionless.
% Thus, it inspired a whole new direction in this field.
Bitcoin represents an important innovation from classical consensus protocols as it is fully open and decentralized.
In the Bitcoin consensus protocol (sometimes called Nakamoto consensus)
participants can join and leave as they wish, and Sybils are handled through the use of \textit{Proof-of-Work} (PoW).

The data structure that keeps track of the state of the system in Bitcoin is a chain of chronologically ordered blocks i.e.,  the blockchain, with each block containing a list of transactions.
To win the right to append a block (and win the block reward), participants compete to solve a computational puzzle i.e.,  a PoW.
They include in their block the solution to that puzzle, the PoW, such that other players can verify its correctness.
This block then initiate a new puzzle to be solved. This process of creating new blocks is called \textit{mining} and participants in this protocol are called \emph{miners}.

If two participants find a solution at roughly the same time, two blocks will be created at the same height in the chain, creating a \textit{fork}, which is problematic as the two blocks can contain conflicting transactions.
To resolve this, each participants will choose one of the two blocks and start creating a new block on top of it by solving the associated PoW.
Whenever a chain becomes longer than the other, participants will abandon the shortest one.
As it is unlikely that two chains will keep the same length for a long time, participants
then reach consensus by following the longest chain rule.

The security of Bitcoin relies on a majority of the mining power (i.e.,  hashing power) in the network following the protocol, whether because they are honest or simply rational.
Taking control of half of the computational power of Bitcoin for only an hour
has a considerable cost (around 670k USD~\cite{crypto51} as of May 2019), although it is with reach of potential adversaries.
This cost depends on the hash rate of the network (i.e.,  the cost of mining) and the price of Bitcoin in USD as once mining is no longer profitable for some miners they are likely to stop mining, reducing the hashing power required to control a majority of the network.

This is one of the reason why Bitcoin's security is so tightly linked to incentives, as when mining is no longer worthwhile the security of the network decreases.
Participation in the network is also rewarded by financial
gain (through block rewards and transaction fees).
The more participants there are, the harder it is to attack the network since the cost for mounting a 51\% attack (where an adversary takes control of more than half of the computational power) increases.
These financial motivations are thus also paramount. 

Since Bitcoin's deployment, many alternative cryptocurrencies that similarly rely on a blockchain have emerged.
The most popular of these is Ethereum~\cite{ethereum}, which differs from Bitcoin in that it provides a more complex scripting
language meaning that rather than processing simple transactions, nodes in the
system execute a script that allows users to perform multitude of functionalities
(so-called \textit{smart contracts}). 

Because PoW consumes a high amount of energy, alternative consensus protocols have been proposed, e.g. Proof-of-Stake (PoS)~\cite{pos-forum}.
Considering PoW as a mechanism that elects a leader based on their computational power (i.e., the participant
who solves the PoW first wins), PoS can be
thought of as a mechanism that elects a leader based on the amount of stake (i.e., coins) that they have in the system.

% \subsection{Terminology}
% \saraha{is there something else to clarify except}
% \subsubsection*{Types of players}
% \noindent

% In traditional mechanism design,
% all parties are assumed to be rational, i.e.,  to behave in a way that maximizes their
% expected utility.
% In Cryptography, parties are either honest or malicious.
% Similarly DS consider good and bad players, the worst type of bad players are Byzantine faults,
% meaning players who behave in a completely arbitrary way.
% In the rest of the paper we will refer to Byzantine players as players who
% behave in an arbitrary way, we will also use the term fully malicious
% or irrational players interchangeably.
% We use rational or selfish players to refer to players that choose their strategy as
% the one that maximize their expected utility.
% We will use altruistic, honest or good players to refer to players that follow
% the protocol.%(with altruistic because honest or good sounds binary)


% Knowledge: in cryptography an adversary will try to learn as much as they can
% in GT knowledge is an underlying assumption.

%\subsubsection*{Terminologies}
% As we've seen, GT, Cryptography and DS use different terminologies to refer to somehow similar concepts.
% We now clarify this terminology.
% In DS,
% Byzantine refer to a process that can deviate arbitrarily from the protocol.
% In Cryptography, this behavior is comparable to that of the adversary.


==> table.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{\linewidth}{!} {%
\begin{tabular} {p{3.5cm}  p{3.5cm}  p{6.5cm} p{3.5cm}  p{6.5cm}}
\toprule \\
    Concept & Assumptions & Description & Flaws & Example, Suggestions and Discussion\\
    \midrule \\
    BAR & Players are Byzantine, Rational, or Honest (altruistic) & & & \\
    $(k,t)$-robustness & Players are Byzantine, Rational, or Honest & This is an extension of NE that consider both coalitions of both rational players (are they incentivize to deviate?) and Byzantine (how the can harm others).& two concepts of immunity and robustness are treated separetely & This model is well suited to study the GT aspects of blockchain consensus protocols.\\
 RPD & Players are rational or Honest & The adversary is rational, does not consider Byzantine adversaries.& Does not consider irrational players & Could be used in Layer 2 since in that case a misbehaving participants will be penalized and the other participant will earn all of its money so a Byzantine adversaries cannot harm honest players more than rational adversaries.\\
 BMG & COnsiders players as Turing Machines \saraha{anything else?} & ? &flaw& could be usefully applied to cryptocurrencies given that many situations are modeled as games involving computations e.g., mining.\\
 Fear factor & rational and byzantine\saraha{double check} & rational players are incentivized to follow the protocol by fear of Byzantine players.&flaw & could be used to argue against the verifier dilemma: 
 some users may be motivated to verify the content of blocks by fear that others will not. \\
 Price of Malice & Rational and Byzantine players & how rational players react to the presence of irrational players. &flaw & could also inspire new measures that quantify the trade-off between blockchain and traditional consensus protocols. Blockchain-based systems are intended to be more scalable as they are meant to handle open par- ticipation, compared to classical consensus that requires the many messages to be exchanged, but in the case of Bitcoin this comes at the price of PoW so there is an incurred economic cost.\\
 Byzantine Price of Anarchy & Rational and Byzantine & quantifies how much an optimal system degrades due to selfish behavior, when malicious players are introduced. &flaw& \\
 Price of Unaccountability & ? & ? &flaw& As differentiating between malicious behavior and genuine latency is hard, especially in PoS systems, the Price of Unaccountability may be a useful to evaluating this. \\
 Hidden actions & ? & don't know what others are doing&flaw & same as above \\
 revelation principle & & &flaw& has been argued to hav ebeen used in system like bitcoin-NG, fruitchain, blockdag etc as they ``reveal'' the rational strategy \saraha{add more}\\
 \hline
\end{tabular}   }
\end{center}
\end{table*}
